Unsupervised Cross-lingual Representation Learning at Scale

This paper shows that pretraining multilingual language models at scale leads to significant performance gains for a wide range of cross-lingual transfer tasks. We train a Transformer-based masked language model on one hundred languages, using more than two terabytes of filtered CommonCrawl data. Our model, dubbed XLM-R, significantly outperforms multilingual BERT (mBERT) on a variety of cross-lingual benchmarks, including +14.6% average accuracy on XNLI, +13% average F1 score on MLQA, and +2.4% F1 score on NER. XLM-R performs particularly well on low-resource languages, improving 15.7% in XNLI accuracy for Swahili and 11.4% for Urdu over previous XLM models. We also present a detailed empirical analysis of the key factors that are required to achieve these gains, including the trade-offs between (1) positive transfer and capacity dilution and (2) the performance of high and low resource languages at scale. Finally, we show, for the first time, the possibility of multilingual modeling without sacrificing per-language performance; XLM-R is very competitive with strong monolingual models on the GLUE and XNLI benchmarks. We will make our code, data and models publicly available.

==> XLMR Paper/content/tables.tex <==



\newcommand{\insertXNLItable}{
    \begin{table*}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{l ccc ccccccccccccccc c}
            \toprule
            {\bf Model} & {\bf D }& {\bf \#M} & {\bf \#lg} & {\bf en} & {\bf fr} & {\bf es} & {\bf de} & {\bf el} & {\bf bg} & {\bf ru} & {\bf tr} & {\bf ar} & {\bf vi} & {\bf th} & {\bf zh} & {\bf hi} & {\bf sw} & {\bf ur} & {\bf Avg}\\
                \midrule
                %\cmidrule(r){1-1}
                %\cmidrule(lr){2-4}
                %\cmidrule(lr){5-19}
                %\cmidrule(l){20-20}
                
                \multicolumn{19}{l}{\it Fine-tune multilingual model on English training set (Cross-lingual Transfer)} \\
                %\midrule
                \midrule
                \citet{lample2019cross} & Wiki+MT & N & 15 & 85.0 & 78.7 & 78.9 & 77.8 & 76.6 & 77.4 & 75.3 & 72.5 & 73.1 & 76.1 & 73.2 & 76.5 & 69.6 & 68.4 & 67.3 & 75.1 \\
                \citet{huang2019unicoder} & Wiki+MT & N & 15 & 85.1 & 79.0 & 79.4 & 77.8 & 77.2 & 77.2 & 76.3 & 72.8 & 73.5 & 76.4 & 73.6 & 76.2 & 69.4 & 69.7 & 66.7 & 75.4 \\
                %\midrule
                \citet{devlin2018bert} & Wiki & N & 102 & 82.1 & 73.8 & 74.3 & 71.1 & 66.4 & 68.9 & 69.0 & 61.6 & 64.9 & 69.5 & 55.8 & 69.3 & 60.0 & 50.4 & 58.0 & 66.3  \\
                \citet{lample2019cross}  & Wiki & N & 100 & 83.7 & 76.2 & 76.6 & 73.7 & 72.4 & 73.0 & 72.1 & 68.1 & 68.4 & 72.0 & 68.2 & 71.5 & 64.5 & 58.0 & 62.4 & 71.3 \\
                \citet{lample2019cross}  & Wiki & 1 & 100 & 83.2 & 76.7 & 77.7 & 74.0 & 72.7 & 74.1 & 72.7 & 68.7 & 68.6 & 72.9 & 68.9 & 72.5 & 65.6 & 58.2 & 62.4 & 70.7 \\
                \bf XLM-R\textsubscript{Base}  & CC & 1 & 100 & 85.8 & 79.7 & 80.7 & 78.7 & 77.5 & 79.6 & 78.1 & 74.2 & 73.8 & 76.5 & 74.6 & 76.7 & 72.4 & 66.5 & 68.3 & 76.2 \\
                \bf XLM-R & CC & 1 & 100 & \bf 89.1 & \bf 84.1 & \bf 85.1 & \bf 83.9 & \bf 82.9 & \bf 84.0 & \bf 81.2 & \bf 79.6 & \bf 79.8 & \bf 80.8 & \bf 78.1 & \bf 80.2 & \bf 76.9 & \bf 73.9 & \bf 73.8 & \bf 80.9 \\
                \midrule
                \multicolumn{19}{l}{\it Translate everything to English and use English-only model (TRANSLATE-TEST)} \\
                \midrule
                BERT-en & Wiki & 1 & 1 & 88.8 & 81.4 & 82.3 & 80.1 & 80.3 & 80.9 & 76.2 & 76.0 & 75.4 & 72.0 & 71.9 & 75.6 & 70.0 & 65.8 & 65.8 & 76.2 \\
                RoBERTa & Wiki+CC & 1 & 1 & \underline{\bf 91.3} & 82.9 & 84.3 & 81.2 & 81.7 & 83.1 & 78.3 & 76.8 & 76.6 & 74.2 & 74.1 & 77.5 & 70.9 & 66.7 & 66.8 & 77.8 \\
                % XLM-en & Wiki & 1 & 1 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0  & 00.0 & 00.0 \\
                \midrule
                \multicolumn{19}{l}{\it Fine-tune multilingual model on each training set (TRANSLATE-TRAIN)} \\
                \midrule 
                \citet{lample2019cross}  & Wiki & N & 100 & 82.9 & 77.6 & 77.9 & 77.9 & 77.1 & 75.7 & 75.5 & 72.6 & 71.2 & 75.8 & 73.1 & 76.2 & 70.4 & 66.5  & 62.4 & 74.2 \\
                \midrule
                \multicolumn{19}{l}{\it Fine-tune multilingual model on all training sets (TRANSLATE-TRAIN-ALL)} \\
                \midrule
                \citet{lample2019cross}$^{\dagger}$ & Wiki+MT & 1 & 15 & 85.0 & 80.8 & 81.3 & 80.3 & 79.1 & 80.9 & 78.3 & 75.6 & 77.6 & 78.5 & 76.0 & 79.5 & 72.9 & 72.8 & 68.5 & 77.8 \\
                \citet{huang2019unicoder} & Wiki+MT & 1 & 15 & 85.6 & 81.1 & 82.3 & 80.9 & 79.5 & 81.4 & 79.7 & 76.8 & 78.2 & 77.9 & 77.1 & 80.5 & 73.4 & 73.8 & 69.6 & 78.5 \\
                %\midrule
                \citet{lample2019cross}  & Wiki & 1 & 100 & 84.5 & 80.1 & 81.3 & 79.3 & 78.6 & 79.4 & 77.5 & 75.2 & 75.6 & 78.3 & 75.7 & 78.3 & 72.1 & 69.2 & 67.7 & 76.9 \\
                \bf XLM-R\textsubscript{Base} & CC & 1 & 100 & 85.4 & 81.4 & 82.2 & 80.3 & 80.4 & 81.3 & 79.7 & 78.6 & 77.3 & 79.7 & 77.9 & 80.2 & 76.1 & 73.1 & 73.0 & 79.1 \\
                \bf XLM-R & CC & 1 & 100 & \bf 89.1 & \underline{\bf 85.1} & \underline{\bf 86.6} & \underline{\bf 85.7} & \underline{\bf 85.3} & \underline{\bf 85.9} & \underline{\bf 83.5} & \underline{\bf 83.2} & \underline{\bf 83.1} & \underline{\bf 83.7} & \underline{\bf 81.5} & \underline{\bf 83.7} & \underline{\bf 81.6} & \underline{\bf 78.0} & \underline{\bf 78.1} & \underline{\bf 83.6} \\
                \bottomrule
            \end{tabular}
            }
            \caption{\textbf{Results on cross-lingual classification.} We report the accuracy on each of the 15 XNLI languages and the average accuracy. We specify the dataset D used for pretraining, the number of models \#M the approach requires and the number of languages \#lg the model handles. Our \xlmr results are averaged over five different seeds. We show that using the translate-train-all approach which leverages training sets from multiple languages, \xlmr obtains a new state of the art on XNLI of $83.6$\% average accuracy. Results with $^{\dagger}$ are from \citet{huang2019unicoder}. %It also outperforms previous methods on cross-lingual transfer.
            \label{tab:xnli}}
        \end{center}
%       \vspace{-0.4cm}
    \end{table*}
}

% Evolution of performance w.r.t number of languages
\newcommand{\insertLanguagesize}{
    \begin{table*}[h!]
    \begin{minipage}{0.49\textwidth}
      \includegraphics[scale=0.4]{content/wiki_vs_cc.pdf}
    \end{minipage}
        \hfill
    \begin{minipage}{0.4\textwidth}
    	\captionof{figure}{\textbf{Distribution of the amount of data (in MB) per language for Wikipedia and CommonCrawl.} The Wikipedia data used in open-source mBERT and XLM is not sufficient for the model to develop an understanding of low-resource languages. The CommonCrawl data we collect alleviates that issue and creates the conditions for a single model to understand text coming from multiple languages. \label{fig:lgs}}
    \end{minipage}
%    \vspace{-0.5cm}
    \end{table*}
}

% Evolution of performance w.r.t number of languages
\newcommand{\insertXLMmorelanguages}{
    \begin{table*}[h!]
    \begin{minipage}{0.49\textwidth}
      \includegraphics[scale=0.4]{content/evolution_languages}
    \end{minipage}
        \hfill
    \begin{minipage}{0.4\textwidth}
    	\captionof{figure}{\textbf{Evolution of XLM performance on SeqLab, XNLI and GLUE as the number of languages increases.} While there are subtlteties as to what languages lose more accuracy than others as we add more languages, we observe a steady decrease of the overall monolingual and cross-lingual performance. \label{fig:lgsunused}}
    \end{minipage}
%    \vspace{-0.5cm}
    \end{table*}
}

\newcommand{\insertMLQA}{
\begin{table*}[h!]
    \begin{center}
        % \scriptsize
        \resizebox{1\linewidth}{!}{
        \begin{tabular}[h]{l cc ccccccc c}
        \toprule
            {\bf Model} & {\bf train} & {\bf \#lgs} & {\bf en} & {\bf es} & {\bf de} & {\bf ar} & {\bf hi} & {\bf vi} & {\bf zh} & {\bf Avg} \\
            \midrule
            BERT-Large$^{\dagger}$ & en & 1 & 80.2 / 67.4 & - & - & - & - & - & - & - \\
            mBERT$^{\dagger}$ & en & 102 & 77.7 / 65.2 & 64.3 / 46.6 & 57.9 / 44.3 & 45.7 / 29.8 & 43.8 / 29.7 & 57.1 / 38.6 & 57.5 / 37.3 & 57.7 / 41.6 \\
            XLM-15$^{\dagger}$ & en & 15 & 74.9 / 62.4 & 68.0 / 49.8 & 62.2 / 47.6 & 54.8 / 36.3 & 48.8 / 27.3 & 61.4 / 41.8 & 61.1 / 39.6 & 61.6 / 43.5 \\
            XLM-R\textsubscript{Base} & en & 100 & 77.1 / 64.6 & 67.4 / 49.6 & 60.9 / 46.7 & 54.9 / 36.6 & 59.4 / 42.9 & 64.5 / 44.7 & 61.8 / 39.3 & 63.7 / 46.3 \\
            \bf XLM-R & en & 100 & \bf 80.6 / 67.8 & \bf 74.1 / 56.0 & \bf 68.5 / 53.6 & \bf 63.1 / 43.5 & \bf 69.2 / 51.6 & \bf 71.3 / 50.9 & \bf 68.0 / 45.4 & \bf 70.7 / 52.7  \\
            \bottomrule
        \end{tabular}
            }
            \caption{\textbf{Results on MLQA question answering} We report the F1 and EM (exact match) scores for zero-shot classification where models are fine-tuned on the English Squad dataset and evaluated on the 7 languages of MLQA. Results with $\dagger$ are taken from the original MLQA paper \citet{lewis2019mlqa}.
            \label{tab:mlqa}}
    \end{center}
\end{table*}
}

\newcommand{\insertNER}{
\begin{table}[t]
    \begin{center}
        % \scriptsize
        \resizebox{1\linewidth}{!}{
        \begin{tabular}[b]{l cc cccc c}
            \toprule
            {\bf Model} & {\bf train} & {\bf \#M} & {\bf en} & {\bf nl} & {\bf es} & {\bf de} & {\bf Avg}\\
            \midrule
            \citet{lample-etal-2016-neural} & each & N & 90.74 & 81.74 & 85.75 & 78.76 & 84.25 \\
            \citet{akbik2018coling} & each & N & \bf 93.18 & 90.44 & - & \bf 88.27 & - \\
            \midrule
            \multirow{2}{*}{mBERT$^{\dagger}$} & each & N & 91.97 & 90.94 & 87.38 & 82.82 & 88.28\\
             & en & 1 & 91.97 & 77.57 & 74.96 & 69.56 & 78.52\\
             \midrule
            \multirow{3}{*}{XLM-R\textsubscript{Base}} & each & N & 92.25 & 90.39 & 87.99 & 84.60 & 88.81\\
             & en & 1 & 92.25 & 78.08 & 76.53 & 69.60 & 79.11\\
             & all & 1 & 91.08 & 89.09 & 87.28 & 83.17 & 87.66 \\
             \midrule
            \multirow{3}{*}{\bf XLM-R} & each & N & 92.92 & \bf 92.53 & \bf 89.72 & 85.81 & 90.24\\
             & en & 1 & 92.92 & 80.80 & 78.64 & 71.40 & 80.94\\
             & all & 1 & 92.00 & 91.60 & 89.52 & 84.60 & 89.43 \\
            \bottomrule
        \end{tabular}
            }
            \caption{\textbf{Results on named entity recognition} on CoNLL-2002 and CoNLL-2003 (F1 score). Results with $\dagger$ are from \citet{wu2019beto}. Note that mBERT and \xlmr do not use a linear-chain CRF, as opposed to \citet{akbik2018coling} and \citet{lample-etal-2016-neural}.
            \label{tab:ner}}
        \end{center}
       \vspace{-0.6cm}
    \end{table}
}


\newcommand{\insertAblationone}{
\begin{table*}[h!]
	\begin{minipage}[t]{0.3\linewidth}
	\begin{center}
          %\includegraphics[width=\linewidth]{content/xlmroberta_transfer_dilution.pdf}
          \includegraphics{content/dilution}
        \captionof{figure}{The transfer-interference trade-off: Low-resource languages benefit from scaling to more languages, until dilution (interference) kicks in and degrades overall performance.}
            \label{fig:transfer_dilution}
        \vspace{-0.2cm}
	\end{center}
    \end{minipage}
    \hfill
	\begin{minipage}[t]{0.3\linewidth}
	\begin{center}
          %\includegraphics[width=\linewidth]{content/xlmroberta_evolution.pdf}
          \includegraphics{content/wikicc}
        \captionof{figure}{Wikipedia versus CommonCrawl: An XLM-7 obtains significantly better performance when trained on CC, in particular on low-resource languages.}
            \label{fig:curse}
	\end{center}
    \end{minipage}
    \hfill
	\begin{minipage}[t]{0.3\linewidth}
	\begin{center}
        % \includegraphics[width=\linewidth]{content/xlmroberta_evolution.pdf}
          \includegraphics{content/capacity}
        \captionof{figure}{Adding more capacity to the model alleviates the curse of multilinguality, but remains an issue for models of moderate size.}
            \label{fig:capacity}
	\end{center}
    \end{minipage}
    \vspace{-0.2cm}
\end{table*}
}


\newcommand{\insertAblationtwo}{
\begin{table*}[h!]
	\begin{minipage}[t]{0.3\linewidth}
        \begin{center}
          %\includegraphics[width=\columnwidth]{content/xlmroberta_alpha_tradeoff.pdf}
          \includegraphics{content/langsampling}
        \captionof{figure}{On the high-resource versus low-resource trade-off: impact of batch language sampling for XLM-100.
        \label{fig:alpha}}
        \end{center}
    \end{minipage}
    \hfill
	\begin{minipage}[t]{0.3\linewidth}
        \begin{center}
          %\includegraphics[width=\columnwidth]{content/xlmroberta_vocab.pdf}
          \includegraphics{content/vocabsize.pdf}
        \captionof{figure}{On the impact of vocabulary size at fixed capacity and with increasing capacity for XLM-100.
        \label{fig:vocab}}
        \end{center}
    \end{minipage}
    \hfill
	\begin{minipage}[t]{0.3\linewidth}
        \begin{center}
          %\includegraphics[width=\columnwidth]{content/xlmroberta_batch_and_tok.pdf}
          \includegraphics{content/batchsize.pdf}
        \captionof{figure}{On the impact of large-scale training, and preprocessing simplification from BPE with tokenization to SPM on raw text data.
        \label{fig:batch}}
        \end{center}
    \end{minipage}
        \vspace{-0.2cm}
\end{table*}
}


% Multilingual vs monolingual
\newcommand{\insertMultiMono}{
    \begin{table}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{l cc ccccccc c}
            \toprule
                {\bf Model} & {\bf D } & {\bf \#vocab} & {\bf en} & {\bf fr} & {\bf de} & {\bf ru} & {\bf zh} & {\bf sw} & {\bf ur} & {\bf Avg}\\
                \midrule
                \multicolumn{11}{l}{\it Monolingual baselines}\\
                \midrule
                \multirow{2}{*}{BERT} & Wiki & 40k & 84.5 & 78.6 & 80.0 & 75.5 & 77.7 & 60.1 & 57.3 & 73.4 \\
                 & CC & 40k & 86.7 & 81.2 & 81.2 & 78.2 & 79.5 & 70.8 & 65.1 & 77.5 \\
                \midrule
                \multicolumn{11}{l}{\it Multilingual models (cross-lingual transfer)}\\
                \midrule
                \multirow{2}{*}{XLM-7} & Wiki & 150k & 82.3 & 76.8 & 74.7 & 72.5 & 73.1 & 60.8 & 62.3 & 71.8 \\
                 & CC & 150k & 85.7 & 78.6 & 79.5 & 76.4 & 74.8 & 71.2 & 66.9 & 76.2 \\
                \midrule
                \multicolumn{11}{l}{\it  Multilingual models (translate-train-all)}\\
                \midrule
                \multirow{2}{*}{XLM-7} & Wiki & 150k & 84.6 & 80.1 & 80.2 & 75.7 & 78 & 68.7 & 66.7 & 76.3 \\
                 & CC & 150k & \bf 87.2 & \bf 82.5 & \bf 82.9 & \bf 79.7 & \bf 80.4 & \bf 75.7 & \bf 71.5 & \bf 80.0 \\ 
                % \midrule
                % XLM (sw,ar) & CC & 60k & N & 2-3 & - & - & - & - & - & 00.0 & - & 00.0 \\
                % XLM (ur,hi,ar) & CC & 60k & N & 2-3 & - & - & - & - & - & - & 00.0 & 00.0 \\
                \bottomrule
            \end{tabular}
            }
            \caption{\textbf{Multilingual versus monolingual models (BERT-BASE).} We compare the performance of monolingual models (BERT) versus multilingual models (XLM) on seven languages, using a BERT-BASE architecture. We choose a vocabulary size of 40k and 150k for monolingual and multilingual models.
            \label{tab:multimono}}
        \end{center}
       \vspace{-0.4cm}
    \end{table}
}

% GLUE benchmark results
\newcommand{\insertGlue}{
    \begin{table}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{l|c|cccccc|c}
            \toprule
                {\bf Model} & {\bf \#lgs} & {\bf MNLI-m/mm} & {\bf QNLI} & {\bf QQP} & {\bf SST} & {\bf MRPC} & {\bf STS-B} & {\bf Avg}\\
                \midrule
                BERT\textsubscript{Large}$^{\dagger}$ & 1 & 86.6/- & 92.3 & 91.3 & 93.2 & 88.0 & 90.0 & 90.2 \\
                XLNet\textsubscript{Large}$^{\dagger}$ & 1 & 89.8/- & 93.9 & 91.8 & 95.6 & 89.2 & 91.8 & 92.0 \\
                RoBERTa$^{\dagger}$ & 1 & 90.2/90.2 & 94.7 & 92.2 & 96.4 & 90.9 & 92.4 & 92.8 \\
                XLM-R & 100 & 88.9/89.0 & 93.8 & 92.3 & 95.0 & 89.5 & 91.2 & 91.8 \\
                \bottomrule
            \end{tabular}
            }
            \caption{\textbf{GLUE dev results.} Results with $^{\dagger}$ are from \citet{roberta2019}.  We compare the performance of \xlmr to BERT\textsubscript{Large}, XLNet and RoBERTa on the English GLUE benchmark.
            \label{tab:glue}}
        \end{center}
       \vspace{-0.4cm}
    \end{table}
}


% Wiki vs CommonCrawl statistics
\newcommand{\insertWikivsCC}{
    \begin{table*}[h]
        \begin{center}
          %\includegraphics[width=\linewidth]{content/wiki_vs_cc.pdf}
          \includegraphics{content/datasize.pdf}
        \captionof{figure}{Amount of data in GiB (log-scale) for the 88 languages that appear in both the Wiki-100 corpus used for mBERT and XLM-100, and the CC-100 used for XLM-R. CC-100 increases the amount of data by several orders of magnitude, in particular for low-resource languages.
        \label{fig:wikivscc}}
        \end{center}
%       \vspace{-0.4cm}
    \end{table*}
}

% Corpus statistics for CC-100
\newcommand{\insertDataStatistics}{
%\resizebox{1\linewidth}{!}{
\begin{table}[h!]
\begin{center}
\small
\begin{tabular}[b]{clrrclrr}
\toprule
\textbf{ISO code} & \textbf{Language} & \textbf{Tokens} (M) & \textbf{Size} (GiB) & \textbf{ISO code} & \textbf{Language} & \textbf{Tokens} (M) & \textbf{Size} (GiB)\\
\cmidrule(r){1-4}\cmidrule(l){5-8}
{\bf af }& Afrikaans & 242 & 1.3 &{\bf  lo }& Lao & 17 & 0.6 \\
{\bf am }& Amharic & 68 & 0.8 &{\bf  lt }& Lithuanian & 1835 & 13.7 \\
{\bf ar }& Arabic & 2869 & 28.0 &{\bf  lv }& Latvian & 1198 & 8.8 \\
{\bf as }& Assamese & 5 & 0.1 &{\bf  mg }& Malagasy & 25 & 0.2 \\
{\bf az }& Azerbaijani & 783 & 6.5 &{\bf  mk }& Macedonian & 449 & 4.8 \\
{\bf be }& Belarusian & 362 & 4.3 &{\bf  ml }& Malayalam & 313 & 7.6 \\
{\bf bg }& Bulgarian & 5487 & 57.5 &{\bf  mn }& Mongolian & 248 & 3.0 \\
{\bf bn }& Bengali & 525 & 8.4 &{\bf  mr }& Marathi & 175 & 2.8 \\
{\bf - }& Bengali Romanized & 77 & 0.5 &{\bf  ms }& Malay & 1318 & 8.5 \\
{\bf br }& Breton & 16 & 0.1 &{\bf  my }& Burmese & 15 & 0.4 \\
{\bf bs }& Bosnian & 14 & 0.1 &{\bf  my }& Burmese & 56 & 1.6 \\
{\bf ca }& Catalan & 1752 & 10.1 &{\bf  ne }& Nepali & 237 & 3.8 \\
{\bf cs }& Czech & 2498 & 16.3 &{\bf  nl }& Dutch & 5025 & 29.3 \\
{\bf cy }& Welsh & 141 & 0.8 &{\bf  no }& Norwegian & 8494 & 49.0 \\
{\bf da }& Danish & 7823 & 45.6 &{\bf  om }& Oromo & 8 & 0.1 \\
{\bf de }& German & 10297 & 66.6 &{\bf  or }& Oriya & 36 & 0.6 \\
{\bf el }& Greek & 4285 & 46.9 &{\bf  pa }& Punjabi & 68 & 0.8 \\
{\bf en }& English & 55608 & 300.8 &{\bf  pl }& Polish & 6490 & 44.6 \\
{\bf eo }& Esperanto & 157 & 0.9 &{\bf  ps }& Pashto & 96 & 0.7 \\
{\bf es }& Spanish & 9374 & 53.3 &{\bf  pt }& Portuguese & 8405 & 49.1 \\
{\bf et }& Estonian & 843 & 6.1 &{\bf  ro }& Romanian & 10354 & 61.4 \\
{\bf eu }& Basque & 270 & 2.0 &{\bf  ru }& Russian & 23408 & 278.0 \\
{\bf fa }& Persian & 13259 & 111.6 &{\bf  sa }& Sanskrit & 17 & 0.3 \\
{\bf fi }& Finnish & 6730 & 54.3 &{\bf  sd }& Sindhi & 50 & 0.4 \\
{\bf fr }& French & 9780 & 56.8 &{\bf  si }& Sinhala & 243 & 3.6 \\
{\bf fy }& Western Frisian & 29 & 0.2 &{\bf  sk }& Slovak & 3525 & 23.2 \\
{\bf ga }& Irish & 86 & 0.5 &{\bf  sl }& Slovenian & 1669 & 10.3 \\
{\bf gd }& Scottish Gaelic & 21 & 0.1 &{\bf  so }& Somali & 62 & 0.4 \\
{\bf gl }& Galician & 495 & 2.9 &{\bf  sq }& Albanian & 918 & 5.4 \\
{\bf gu }& Gujarati & 140 & 1.9 &{\bf  sr }& Serbian & 843 & 9.1 \\
{\bf ha }& Hausa & 56 & 0.3 &{\bf  su }& Sundanese & 10 & 0.1 \\
{\bf he }& Hebrew & 3399 & 31.6 &{\bf  sv }& Swedish & 77.8 & 12.1 \\
{\bf hi }& Hindi & 1715 & 20.2 &{\bf  sw }& Swahili & 275 & 1.6 \\
{\bf - }& Hindi Romanized & 88 & 0.5 &{\bf  ta }& Tamil & 595 & 12.2 \\
{\bf hr }& Croatian & 3297 & 20.5 &{\bf  - }& Tamil Romanized & 36 & 0.3 \\
{\bf hu }& Hungarian & 7807 & 58.4 &{\bf  te }& Telugu & 249 & 4.7 \\
{\bf hy }& Armenian & 421 & 5.5 &{\bf  - }& Telugu Romanized & 39 & 0.3 \\
{\bf id }& Indonesian & 22704 & 148.3 &{\bf  th }& Thai & 1834 & 71.7 \\
{\bf is }& Icelandic & 505 & 3.2 &{\bf  tl }& Filipino & 556 & 3.1 \\
{\bf it }& Italian & 4983 & 30.2 &{\bf  tr }& Turkish & 2736 & 20.9 \\
{\bf ja }& Japanese & 530 & 69.3 &{\bf  ug }& Uyghur & 27 & 0.4 \\
{\bf jv }& Javanese & 24 & 0.2 &{\bf  uk }& Ukrainian & 6.5 & 84.6 \\
{\bf ka }& Georgian & 469 & 9.1 &{\bf  ur }& Urdu & 730 & 5.7 \\
{\bf kk }& Kazakh & 476 & 6.4 &{\bf  - }& Urdu Romanized & 85 & 0.5 \\
{\bf km }& Khmer & 36 & 1.5 &{\bf  uz }& Uzbek & 91 & 0.7 \\
{\bf kn }& Kannada & 169 & 3.3 &{\bf  vi }& Vietnamese & 24757 & 137.3 \\
{\bf ko }& Korean & 5644 & 54.2 &{\bf  xh }& Xhosa & 13 & 0.1 \\
{\bf ku }& Kurdish (Kurmanji) & 66 & 0.4 &{\bf  yi }& Yiddish & 34 & 0.3 \\
{\bf ky }& Kyrgyz & 94 & 1.2 &{\bf  zh }& Chinese (Simplified) & 259 & 46.9 \\
{\bf la }& Latin & 390 & 2.5 &{\bf  zh }& Chinese (Traditional) & 176 & 16.6 \\

\bottomrule
\end{tabular}
\caption{\textbf{Languages and statistics of the CC-100 corpus.} We report the list of 100 languages and include the number of tokens (Millions) and the size of the data (in GiB) for each language. Note that we also include romanized variants of some non latin languages such as Bengali, Hindi, Tamil, Telugu and Urdu.\label{tab:datastats}}
\end{center}
\end{table}
%}
}


% Comparison of parameters for different models
\newcommand{\insertParameters}{
    \begin{table*}[h!]
        \begin{center}
            % \scriptsize
            %\resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{lrcrrrrrc}
            \toprule
                \textbf{Model} & \textbf{\#lgs} & \textbf{tokenization} & \textbf{L} & \textbf{$H_{m}$} & \textbf{$H_{ff}$} & \textbf{A} & \textbf{V} & \textbf{\#params}\\
                \cmidrule(r){1-1}
                \cmidrule(lr){2-3}
                \cmidrule(lr){4-8}
                \cmidrule(l){9-9}
                % TODO: rank by number of parameters
                BERT\textsubscript{Base} & 1 & WordPiece & 12 & 768 & 3072 & 12 & 30k & 110M \\
                BERT\textsubscript{Large} & 1 & WordPiece & 24 & 1024 & 4096 & 16 & 30k & 335M \\
                mBERT & 104 & WordPiece & 12 & 768 & 3072 & 12 & 110k & 172M \\
                RoBERTa\textsubscript{Base} & 1 & bBPE & 12 & 768 & 3072 & 8 & 50k & 125M \\
                RoBERTa & 1 & bBPE & 24 & 1024 & 4096 & 16 & 50k & 355M \\
                XLM-15 & 15 & BPE & 12 & 1024 & 4096 & 8 & 95k & 250M \\
                XLM-17 & 17 & BPE & 16 & 1280 & 5120 & 16 & 200k & 570M \\
                XLM-100 & 100 & BPE & 16 & 1280 & 5120 & 16 & 200k & 570M \\
                Unicoder & 15 & BPE & 12 & 1024 & 4096 & 8 & 95k & 250M \\
                \xlmr\textsubscript{Base} & 100 & SPM & 12 & 768 & 3072 & 12 & 250k & 270M \\
                \xlmr & 100 & SPM & 24 & 1024 & 4096 & 16 & 250k & 550M \\
                GPT2 & 1 & bBPE & 48 & 1600 & 6400 & 32 & 50k & 1.5B \\
                wide-mmNMT & 103 & SPM & 12 & 2048 & 16384 & 32 & 64k & 3B \\
                deep-mmNMT & 103 & SPM & 24 & 1024 & 16384 & 32 & 64k & 3B \\
                T5-3B & 1 & WordPiece & 24 & 1024 & 16384 & 32 & 32k & 3B \\
                T5-11B & 1 & WordPiece & 24 & 1024 & 65536 & 32 & 32k & 11B \\
                % XLNet\textsubscript{Large}$^{\dagger}$ & 1 & 89.8/- & 93.9 & 91.8 & 95.6 & 89.2 & 91.8 & 92.0 \\
                % RoBERTa$^{\dagger}$ & 1 & 90.2/90.2 & 94.7 & 92.2 & 96.4 & 90.9 & 92.4 & 92.8 \\
                % XLM-R & 100 & 88.4/88.5 & 93.1 & 92.2 & 95.1 & 89.7 & 90.4 & 91.5 \\
                \bottomrule
            \end{tabular}
            %}
            \caption{\textbf{Details on model sizes.}
            We show the tokenization used by each Transformer model, the number of layers L, the number of hidden states of the model $H_{m}$, the dimension of the feed-forward layer $H_{ff}$, the number of attention heads A, the size of the vocabulary V and the total number of parameters \#params. 
            For Transformer encoders, the number of parameters can be approximated by $4LH_m^2 + 2LH_m H_{ff} + VH_m$.
            GPT2 numbers are from \citet{radford2019language}, mm-NMT models are from the work of \citet{arivazhagan2019massively} on massively multilingual neural machine translation (mmNMT), and T5 numbers are from \citet{raffel2019exploring}. While \xlmr is among the largest models partly due to its large embedding layer, it has a similar number of parameters than XLM-100, and remains significantly smaller that recently introduced Transformer models for multilingual MT and transfer learning. While this table gives more hindsight on the difference of capacity of each model, note it does not highlight other critical differences between the models. 
            \label{tab:parameters}}
        \end{center}
       \vspace{-0.4cm}
    \end{table*}
}
